CV4Code: Sourcecode Understanding via Visual Code Representations

We present CV4Code, a compact and effective computer vision method for sourcecode understanding. Our method leverages the contextual and the structural information available from the code snippet by treating each snippet as a two-dimensional image, which naturally encodes the context and retains the underlying structural information through an explicit spatial representation. To codify snippets as images, we propose an ASCII codepoint-based image representation that facilitates fast generation of sourcecode images and eliminates redundancy in the encoding that would arise from an RGB pixel representation. Furthermore, as sourcecode is treated as images, neither lexical analysis (tokenisation) nor syntax tree parsing is required, which makes the proposed method agnostic to any particular programming language and lightweight from the application pipeline point of view. CV4Code can even featurise syntactically incorrect code which is not possible from methods that depend on the Abstract Syntax Tree (AST). We demonstrate the effectiveness of CV4Code by learning Convolutional and Transformer networks to predict the functional task, i.e. the problem it solves, of the source code directly from its two-dimensional representation, and using an embedding from its latent space to derive a similarity score of two code snippets in a retrieval setup. Experimental results show that our approach achieves state-of-the-art performance in comparison to other methods with the same task and data configurations. For the first time we show the benefits of treating sourcecode understanding as a form of image processing task.

==> fig/activation_maps.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{fig/activation_maps.png}
    \caption{Average activation map across channels (cropped to fit the space). From left to right, C++, Java and Python submissions to the same programming problem (p00001) respectively. Gaussian filter ($\sigma=1$) is used to smooth the heatmap. }
    \label{fig:activation_maps}
\end{figure*}


==> tab/resnet_config.tex <==
\renewcommand{\arraystretch}{1.05}
\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c|c}
    \hline
        \textbf{Layer name} & \textbf{Output size} & \textbf{Kernel} & \textbf{Stride} \\
    \hline
    \hline
        conv0 & $48\times 48\times 16$ & $3\times 3$, 16 & 2\\
    \hline
        max\_pool & $24\times 24\times 16$ & $3\times 3$ & 2\\
    \hline
        conv1 & $12\times 12\times 64$ & $\begin{bmatrix} 3\times 3, 64 \\ 3\times 3, 64 \end{bmatrix} \times 2$ & 2 \\
    \hline
        conv2 & $6\times 6\times 128$ & $\begin{bmatrix} 3\times 3, 128\\ 3\times 3, 128 \end{bmatrix} \times 2$ & 2\\
    \hline
        conv3 & $6\times 6\times 256$ & $\begin{bmatrix} 3\times 3, 256\\ 3\times 3, 256\end{bmatrix} \times 2$ & 1\\
    \hline
        max\_pool & 256 & $6\times6$ & 6\\
    \hline
        fc & 128 & $256 \times 128$ & - \\
    \hline
        AAM-Softmax & $237$ & $128\times 237$ & -\\
    \hline
    \end{tabular}
    \caption{CV4Code-ResNet model configuration. \#params=3.25M.}
    \label{tab:resnet_configuration}
\end{table}

==> tab/similarity_language_ablation.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{c|c|c}
    \hline
       \multirow{2}{*}{\textbf{Language}} & \multicolumn{2}{|c}{\textbf{mAP@R}} \\
         & Known & Unknown  \\
        \hline\hline
        Mixed & 0.766 & 0.644 \\
        C++ & 0.830 & 0.691 \\
        Python & 0.763 & 0.676 \\
    \hline
    \end{tabular}
    \caption{CV4Code-generic code similarity evaluation results. Unknown and known datasets the same used in \ref{tab:code_similarity_results}. Mixed: all languages; C++: only C++, 5228 known samples, 5559 unknown samples; Python: only Python, 2832 known samples and 2438 unknown samples. }
    \label{tab:similarity_language_ablation}
\end{table}
